Bridging the Training-Inference Gap in LLMs by Leveraging Self-Generated Tokens

Language models are often trained to maximize the likelihood of the next token given past tokens in the training dataset. However, during inference time, they are utilized differently, generating text sequentially and auto-regressively by using previously generated tokens as input to predict the next one. Marginal differences in predictions at each step can cascade over successive steps, resulting in different distributions from what the models were trained for and potentially leading to unpredictable behavior. This paper proposes two simple approaches based on model own generation to address this discrepancy between the training and inference time. Our first approach is Batch-Scheduled Sampling, where, during training, we stochastically choose between the ground-truth token from the dataset and the model's own generated token as input to predict the next token. This is done in an offline manner, modifying the context window by interleaving ground-truth tokens with those generated by the model. Our second approach is Reference-Answer-based Correction, where we explicitly incorporate a self-correction capability into the model during training. This enables the model to effectively self-correct the gaps between the generated sequences and the ground truth data without relying on an external oracle model. By incorporating our proposed strategies during training, we have observed an overall improvement in performance compared to baseline methods, as demonstrated by our extensive experiments using summarization, general question-answering, and math question-answering tasks.

==> tex_file/_unused_02_related_work.tex <==
\section{Related Work}
%\TODO{place it here or after intro?}

% old
% Teacher forcing is a widely used training strategy in sequence generation tasks, where the model is trained to predict the next token in a sequence using the previous tokens from the training data as input. This approach accelerates convergence and improves the quality of generated sequences during training. However, a significant drawback of teacher forcing is the discrepancy it creates between training and inference time. During inference, the model must rely on its own predictions as input for subsequent steps, which can lead to error propagation and a drop in performance if the model encounters sequences that diverge from its training conditions.

% To address these limitations, student forcing has emerged as an alternative approach that bridges the gap between training and inference. In student forcing, the model is gradually exposed to its own generated tokens during training, thus more closely simulating the inference scenario. This technique employs methods such as scheduled sampling, where the model uses a mix of true and generated tokens based on a predefined schedule. By fostering a smoother transition from training to inference, student forcing aims to enhance the model's robustness and reduce the performance gap. Recent studies highlight the effectiveness of student forcing in generating more coherent and contextually relevant outputs, demonstrating its potential to improve generalization in sequence generation tasks.

% \TODO{rewrite the first part and polish the second}

Teacher forcing is a widely used training strategy in sequence generation tasks~\citep{ouyang2022training, chung2024scaling}, where the model is trained to predict the next token based on the preceding tokens from the training data. 
% This approach accelerates convergence and improves the quality of generated sequences during training. 
One drawback of teacher forcing is the discrepancy it creates between training and inference time, commonly referred to as exposure bias~\citep{bengio2015scheduled, ranzato2015sequence, schmidt2019generalization, he2019quantifying}. During inference, the model must rely on its own predictions as input for subsequent steps, which can lead to error accumulation and degraded performance especially when the generated sequences deviate from the conditions encountered during training.


To address this limitation, various methods have been proposed to mitigate distribution shift, such as generative adversarial training~\citep{yu2017seqgan, rajeswar2017adversarial, guo2018long, nie2018relgan} or inverse reinforcement learning~\citep{jaques2017tuning, shi2018toward, keneshloo2019deep}. However, those methods can suffer from the training instability, making them difficult to integrate into transformer-based large language models. Student forcing has emerged as an alternative approach where the model is gradually exposed to its own generated tokens during training, thus more closely simulating the condition of inference~\citep{bengio2015scheduled, professorForcing2016}. By fostering a smoother transition from training to inference, student forcing aims to enhance robustness and reduce distribution shift. Recent studies highlight the effectiveness of student forcing in generating more coherent and contextually relevant outputs~\citep{goyaldifferentiable2017, li2020improvingtext}, demonstrating its potential to improve generalization in sequence generation tasks.


Another line of work focuses on self-improvement in language models~\citep{welleck2022generating}. One common approach is to prompt the LLM to generate self-criticism or reflection after providing an initial response to a question by specified query template. This feedback is then used to generate a new response~\citep{shinn2023reflexion, kim2024language, madaan2024self}. However, recent studies suggest that such prompting-based self-improvement may lead to a performance drop~\citep{huang2023large, tyen2023llms, kamoi2024can}. Beyond prompting, other works involve training a new separate model to correct or improve the response of the original model~\citep{akyurek2023rl4f, havrilla2024glore}, which does not improve the original model or mitigate its training-inference gap issue. Some other methods can boost performance remarkably with supervision from advanced models~\citep{pan2023automatically, agarwal2023gkd, qu2024recursive} but those settings are different from ours where no external feedback is available.

% \textbf{Self-correction in language model}. Self-correction capability enables the LLM to improve the quality of generation or fix the error iteratively based on the self-generated correction or guidance~\citep{welleck2022generating, kumar2024training}, which can also facilitate to narrow the gap between expert response in training and model-generated response in inference. While previous works demonstrate that the supervision from advanced models can boost the performance~\citep{pan2023automatically, agarwal2023gkd}, the existing correction methods still struggle without any external feedback~\citep{kamoi2024can}. One direction of self-correction is to prompt the LLM to generate the feedback or reflection itself for the generated response~\citep{ shinn2023reflexion, kim2024language, madaan2024self}, recent studies draw a contradictory conclusion that such prompting-based self-correction may learn to a performance drop~\citep{huang2023large, tyen2023llms, kamoi2024can}. Beyond simple prompting, several works propose to correct the model by multi-turn dialogue with feedback from oracle model or self-generated revision~\citep{qu2024recursive} or train a separate correction model~\citep{akyurek2023rl4f, havrilla2024glore}. However, these methods either show only modest performance improvements or require an additional correction model during deployment, which fails to truly reduce the training-inference gap of the original model.
